Entanglement detection

How can one prove that a given state is entangled? In this paper we review different methods that have been proposed for entanglement detection. We first explain the basic elements of entanglement theory for two or more particles and then entanglement verification procedures such as Bell inequalities, entanglement witnesses, the determination of nonlinear properties of a quantum state via measurements on several copies, and spin squeezing inequalities. An emphasis is given on the theory and application of entanglement witnesses. We also discuss several experiments, where some of the presented methods have been implemented.

==> kieselexp.tex <==
\subsection{Experimental generation of cluster states}
\label{clusterexp}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now we describe an experiment from K.~Chen et 
al.~\cite{chen-2007-99},
where a four-qubit cluster state has been prepared and a stabilizer witness 
has been used.\footnote{At the same time, a similar 
experiment has been performed by Vallone et al.~\cite{TwoPhotonClusterState}.} 
This experiment used hyper-entanglement of photons for the 
creation of the cluster state \cite{Kwiathyper}. This means that several degrees 
of freedom of each photon are used to carry the entanglement, in the given 
experiment, each photon represented two qubits, one polarization qubit and 
one spatial qubit. This technique is becoming more and more important in
multi-photon experiments as it allows to extend the Hilbert space significantly 
\cite{barreiro-2005-95,schuck:190501,kwiatnatphys,vallonenewhyper}.
Quite recently, this technique has been used to realize a ten-qubit GHZ state with
five photons \cite{gao-2008}.

\begin{figure}[t]
\centerline{\includegraphics[width=0.5\columnwidth]{hyperentangledsetup.eps}}
\caption{(a) Setup for the generation of four-qubit cluster states using two 
photons and hyper-entanglement. (b) Required setups for the measurement of the 
polarization qubit and the spatial qubit of one photon. See the text for further
details. Figure is taken from Ref.~\cite{chen-2007-99}.
\label{hypersetup}
}
\end{figure}

The setup of the experiment is shown in Fig.~\ref{hypersetup}. A UV laser 
pulse passes two times through two combined BBO crystals. This leads either 
to emission of $\ket{H_A H_B} + \ket{V_A V_B}$ in the upward direction 
(modes $L_A, L_B$) or to emission of $\ket{H_A H_B} - \ket{V_A V_B}$  
in the downwards direction, i.e., modes $R_A, R_B$. Here, $H$ and $V$ denote horizontal 
and vertical polarization. If the photons overlap perfectly at the beamsplitters $BS_1$ 
and $BS_2,$ the state will be a superposition
\be
\ket{\psi} = \frac{1}{2}
\big[
(\ket{H_A H_B} + \ket{V_A V_B}) \ket{L_A L_B}
+
e^{i \phi}
(\ket{H_A H_B} - \ket{V_A V_B}) \ket{R_A R_B}
\big].
\ee
By adjusting the concave mirror, $\phi = 0$ can be obtained. 
Then the state is equivalent to  the cluster state 
$\ket{\psi}=(\ket{0000}+\ket{0011}+\ket{1100} - \ket{1111}),$ 
if the replacements $\ket{H/V}\mapsto \ket{0/1}$ and 
$\ket{L/R}\mapsto \ket{0/1}$ are done. 
%For later convenience, 
%the qubits are also reordered, such that the polarization
%of the first (second) photon denotes the first (second) qubit, 
%while the spatial mode of the first (second) photon denotes 
%the fourth (third) qubit. 
Since only two photons are 
required, the count rate in the present experiment is 
around $1.2 \cdot 10^4$ per second, which is about four 
orders of magnitude higher than in experiments which produced  
the same cluster state using four photons \cite{PhysRevLett.95.210502,walther-2005-434}.

In order to measure the state, the elements as in 
Fig.~\ref{hypersetup}(b) have been used. A measurement without 
any beamsplitter as in (i) first reads out whether the photon 
is in $L/R$ and also the polarization of the photon. Hence 
it can be used to measure $Z_{\rm spat}X_{\rm pol}$ at one 
photon. Using a beamsplitter as in (ii) leads to a Hadamard 
transformation on the spatial modes, such that 
$X_{\rm spat} Z_{\rm pol}$ can be measured. 
%A configuration as in (iii) may be used to measure
%$Z_{\rm spat} Z_{\rm pol}.$
The problem is that such a setup is sensitive to small 
path length changes, hence it requires a significant 
amount of adjustment and is only stable short 
timescales.\footnote{Only recently, using a Sagnac-like 
interferometer, stable interferometers for this problem have 
been introduced \cite{gao-2008}.}
Therefore, despite of the high counting rate, an analysis 
of the state should require only few measurements.

Therefore, one can use the witness
\be
\mathcal{W}= 2\eins - \frac{1}{2}
(
X_1 X_2 \eins_3 Z_4+
X_1 X_1 Z_3 \eins_4 +
\eins_1 \eins_2 Z_3 Z_4+
\eins_1 Z_2 X_3 X_4 +
Z_1 \eins_2 X_3 X_4 +
Z_1 Z_2 \eins_3 \eins_4
)
\ee 
which is just the witness from Eq.~(\ref{CN}) adapted to the form of the 
cluster state used here. This witness can be measured with the settings 
$X_1 X_2 Z_3 Z_4$ and $Z_1 Z_2 X_3 X_4$. 
This corresponds to the setups in  Fig.~\ref{hypersetup}b (i) 
and (ii). The experimental data give 
\be
\mean{W} = -0.766\pm 0.004 \mbox{ and } F \geq  \frac{1-\mean{W}}{2} =0.883 \pm 0.002, 
\ee
clearly confirming the four-qubit entanglement. Furthermore, this cluster state has 
then been used to demonstrate two-qubit gates.

Finally, let us add that due to the hyper-entanglement the four qubits 
are not spatially separated, hence the entanglement refers to different degrees of 
freedom, and not different particles. Interestingly, of one is interested in 
the entanglement between the hyper-entangled particles, stabilizer witnesses 
can again be used \cite{vallone-2008}.

%%%%%%%%%%%%%%

